The temporal changes of the pulsational periods of the pre-white dwarf PG 1159-035

PG 1159-035, a pre-white dwarf with T=140000 K, is the prototype of the PG1159 spectroscopic class and the DOV pulsating class. Changes in the star cause variations in its oscillation periods. The measurement of temporal change in the oscillation periods, dP/dt, allows us to estimate directly rates of stellar evolutionary changes, such as the cooling rate and the envelope contraction rate, providing a way to test and refine evolutionary models for pre-white dwarf pulsating stars. We measured 27 pulsation modes period changes. The periods varied at rates of between 1 and 100 ms/yr, and several can be directly measured with a relative standard uncertainty below 10%. For the 516.0 s mode (the highest in amplitude) in particular, not only the value of dP/dt can be measured directly with a relative standard uncertainty of 2%, but the second order period change, d(dP/dt)/dt, can also be calculated reliably. By using the (O-C) method we refined the dP/dt and estimated the d(dP/dt)/dt for six other pulsation periods. As a first application, we calculated the change in the PG 1559-035 rotation period, dP_rot/dt = -2.13*10^{-6} s/s, the envelope contraction rate dR/dt = -2.2*10^{-13} solar radius/s, and the cooling rante dT/dt = -1.42*10^{-3} K/s.

==> 9118tb3.tex <==
% Tabela com as amplitudes para cada ano.
\begin{tabular}{cccccc} \hline \hline 
Mode  & 1983 & 1985 & 1989 & 1993 & 2002 \\
 (s)      &        &         &        &         &      \\ \hline
          &        &         &        &         &      \\ 
 376.0   &  $ 0.72 \pm 0.13$ & $ 0.35 \pm 0.19$ &   ---  &   ---  &   ---  \\
 387.4   &    ---  &   ---  & $ 0.30 \pm 0.05$ &   ---  & $ 0.43 \pm 0.09$ \\
 390.3   &  $ 1.77 \pm 0.13$ &   ---  & $ 1.01 \pm 0.05$ &   ---  & $ 0.22 \pm 0.09$ \\
 390.8   &    ---  &   ---  &   ---  & $ 0.28 \pm 0.07$ & $ 0.15 \pm 0.09$ \\
 397.2   &    ---  & $ 0.49 \pm 0.17$ &   ---  &   ---  & $ 0.33 \pm 0.09$ \\
 399.0   &    ---  &   ---  & $ 0.37 \pm 0.05$ &   ---  & $ 0.66 \pm 0.09$ \\
 400.0   &    ---  &   ---  & $ 1.42 \pm 0.05$ & $ 0.79 \pm 0.07$ & $ 0.61 \pm 0.09$ \\
 401.6   &    ---  &   ---  &   ---  &   ---  & $ 0.38 \pm 0.09$ \\
 412.0   &    ---  &   ---  & $ 0.60 \pm 0.05$ &   ---  & $ 0.64 \pm 0.09$ \\
 414.3   &    ---  &   ---  & $ 0.65 \pm 0.05$ & $ 0.56 \pm 0.07$ & $ 0.70 \pm 0.09$ \\
 415.5   &    ---  & $ 0.81 \pm 0.18$ & $ 1.19 \pm 0.05$ &   ---  & $ 0.51 \pm 0.09$ \\
 422.5   &  $ 2.36 \pm 0.13$ &   ---  &   ---  & $ 1.82 \pm 0.07$ & $ 1.64 \pm 0.09$ \\
 426.2   &    ---  &   ---  &   ---  & $ 0.80 \pm 0.07$ & $ 0.98 \pm 0.09$ \\
 427.5   &    ---  &   ---  & $ 1.92 \pm 0.05$ & $ 0.85 \pm 0.07$ & $ 0.16 \pm 0.09$ \\
 430.3   &  $ 0.61 \pm 0.14$ &   ---  &   ---  &   ---  & $ 0.24 \pm 0.09$ \\
 434.2   &    ---  & $ 0.88 \pm 0.19$ &   ---  &   ---  & $ 0.48 \pm 0.09$ \\
 436.5   &    ---  &   ---  & $ 0.41 \pm 0.05$ & $ 0.72 \pm 0.07$ & $ 0.39 \pm 0.09$ \\
 439.2   &    ---  &   ---  & $ 0.49 \pm 0.05$ & $ 0.61 \pm 0.07$ & $ 0.60 \pm 0.09$ \\
 440.6   &    ---  &   ---  & $ 1.05 \pm 0.05$ & $ 1.26 \pm 0.07$ & $ 0.72 \pm 0.09$ \\
 451.5   &  $ 4.54 \pm 0.15$ & $ 2.72 \pm 0.21$ & $ 3.70 \pm 0.05$ & $ 3.93 \pm 0.07$ & $ 3.39 \pm 0.09$ \\
 452.4   &  $ 2.78 \pm 0.15$ & $ 1.37 \pm 0.20$ & $ 3.36 \pm 0.05$ & $ 2.80 \pm 0.07$ & $ 2.78 \pm 0.09$ \\
 453.2   &  $ 1.41 \pm 0.14$ &   ---  &   ---  & $ 1.56 \pm 0.07$ & $ 1.47 \pm 0.09$ \\
 493.7   &  $ 5.47 \pm 0.16$ & $ 3.00 \pm 0.22$ & $ 3.47 \pm 0.05$ & $ 2.75 \pm 0.07$ &   ---  \\
 494.8   &  $ 2.34 \pm 0.15$ &   ---  & $ 0.46 \pm 0.05$ & $ 0.72 \pm 0.07$ &   ---  \\
 511.9   &    ---  &   ---  & $ 0.29 \pm 0.05$ & $ 0.59 \pm 0.07$ &   ---  \\
 515.0   &  $ 0.91 \pm 0.14$ & $ 1.21 \pm 0.20$ &   ---  & $ 0.58 \pm 0.07$ & $ 0.69 \pm 0.09$ \\
 516.0   &  $ 8.76 \pm 0.16$ & $ 7.45 \pm 0.24$ & $ 6.17 \pm 0.06$ & $ 5.91 \pm 0.08$ & $ 7.25 \pm 0.09$ \\
 517.1   &  $ 1.30 \pm 0.15$ & $ 3.01 \pm 0.22$ & $ 3.89 \pm 0.05$ & $ 4.26 \pm 0.08$ &   ---  \\
 518.2   &    ---  &   ---  & $ 3.58 \pm 0.06$ & $ 3.12 \pm 0.08$ & $ 1.71 \pm 0.09$ \\
 526.4   &    ---  &   ---  & $ 0.16 \pm 0.05$ &   ---  & $ 0.77 \pm 0.09$ \\
 536.9   &  $ 1.01 \pm 0.14$ &   ---  & $ 1.41 \pm 0.06$ & $ 0.52 \pm 0.07$ & $ 1.16 \pm 0.10$ \\
 538.1   &  $ 4.48 \pm 0.16$ &   ---  & $ 3.82 \pm 0.05$ &   ---  & $ 2.98 \pm 0.09$ \\
 539.3   &  $ 5.93 \pm 0.16$ & $ 4.48 \pm 0.20$ & $ 5.37 \pm 0.06$ & $ 7.47 \pm 0.08$ &   ---  \\
 540.9   &    ---  &   ---  &   ---  & $ 0.55 \pm 0.07$ & $ 0.23 \pm 0.09$ \\
 544.3   &    ---  &   ---  &   ---  & $ 0.41 \pm 0.07$ & $ 0.63 \pm 0.10$ \\
 557.1   &    ---  &   ---  & $ 3.14 \pm 0.05$ & $ 0.69 \pm 0.08$ & $ 1.04 \pm 0.09$ \\
 558.4   &    ---  &   ---  & $ 2.49 \pm 0.05$ & $ 1.51 \pm 0.08$ & $ 2.22 \pm 0.09$ \\
 559.7   &    ---  &   ---  & $ 0.84 \pm 0.05$ & $ 1.38 \pm 0.08$ & $ 0.56 \pm 0.09$ \\
 561.9   &  $ 1.21 \pm 0.15$ &   ---  &   ---  & $ 0.43 \pm 0.08$ & $ 0.55 \pm 0.09$ \\
 641.4   &    ---  &   ---  & $ 1.03 \pm 0.05$ & $ 0.35 \pm 0.07$ &   ---  \\
 644.9   &    ---  & $ 1.75 \pm 0.24$ & $ 0.87 \pm 0.05$ &   ---  &   ---  \\
 668.5   &    ---  &   ---  & $ 0.35 \pm 0.05$ &   ---  & $ 0.35 \pm 0.09$ \\
 685.8   &    ---  &   ---  & $ 0.17 \pm 0.05$ & $ 0.39 \pm 0.07$ &   ---  \\
 689.7   &    ---  &   ---  & $ 0.51 \pm 0.05$ & $ 0.60 \pm 0.07$ &   ---  \\
 705.8   &    ---  & $ 0.76 \pm 0.19$ & $ 0.75 \pm 0.05$ &   ---  &   ---  \\
 727.0   &    ---  &   ---  & $ 0.72 \pm 0.05$ &   ---  & $ 0.60 \pm 0.09$ \\
 729.6   &    ---  &   ---  & $ 0.29 \pm 0.05$ & $ 0.36 \pm 0.07$ &   ---  \\
 731.6   &    ---  &   ---  & $ 0.98 \pm 0.05$ & $ 0.55 \pm 0.07$ & $ 0.34 \pm 0.09$ \\
 755.3   &    ---  &   ---  & $ 0.31 \pm 0.05$ & $ 0.33 \pm 0.07$ &   ---  \\
 812.5   &    ---  & $ 0.73 \pm 0.18$ & $ 0.41 \pm 0.05$ &   ---  &   ---  \\
 819.7   &  $ 1.40 \pm 0.14$ &   ---  & $ 0.81 \pm 0.05$ & $ 0.65 \pm 0.07$ &   ---  \\
 842.8   &  $ 2.28 \pm 0.14$ &   ---  & $ 0.91 \pm 0.05$ &   ---  &   ---  \\
 861.7   &    ---  & $ 1.09 \pm 0.18$ &   ---  & $ 0.72 \pm 0.07$ &   ---  \\
 877.6   &    ---  &   ---  &   ---  & $ 0.30 \pm 0.07$ & $ 0.53 \pm 0.09$ \\

        &      &      &      &      &      \\ \hline
 \end{tabular}



==> 9118tb4.tex <==
% Tabela com os perídos para cada ano.
\begin{tabular}{cccccc} \hline \hline 
Year    & 1983 & 1985 & 1989 & 1993 & 2002 \\
BCT     & $ 244\,5346.0+$      & $ 244\,6147.0+$       & $ 244\,7593.0+$      &  $ 244\,9065.0+$      & $ 245\,2410.0+$    \\ \hline
Period (s)   &        &         &        &         &      \\ 
 376.0   &  $0.87548 \pm 0.00038$ & $0.66449 \pm 0.00079$ &   ---  &   ---  &   ---  \\
 387.4   &    ---  &   ---  & $0.33622 \pm 0.00028$ &   ---  & $0.63362 \pm 0.00030$ \\
 390.3   &  $0.87395 \pm 0.00016$ &   ---  & $0.33753 \pm 0.00009$ &   ---  & $0.63347 \pm 0.00059$ \\
 390.8   &    ---  &   ---  &   ---  & $0.92851 \pm 0.00034$ & $0.63559 \pm 0.00090$ \\
 397.2   &    ---  & $0.66570 \pm 0.00055$ &   ---  &   ---  & $0.63552 \pm 0.00042$ \\
 399.0   &    ---  &   ---  & $0.33756 \pm 0.00023$ &   ---  & $0.63368 \pm 0.00020$ \\
 400.0   &    ---  &   ---  & $0.33522 \pm 0.00006$ & $0.92791 \pm 0.00012$ & $0.63537 \pm 0.00022$ \\
 401.6   &    ---  &   ---  &   ---  &   ---  & $0.63608 \pm 0.00037$ \\
 412.0   &    ---  &   ---  & $0.33584 \pm 0.00015$ &   ---  & $0.63361 \pm 0.00022$ \\
 414.3   &    ---  &   ---  & $0.33513 \pm 0.00015$ & $0.92697 \pm 0.00018$ & $0.63441 \pm 0.00020$ \\
 415.5   &    ---  & $0.66172 \pm 0.00037$ & $0.33537 \pm 0.00008$ &   ---  & $0.63412 \pm 0.00027$ \\
 422.5   &  $0.87207 \pm 0.00013$ &   ---  &   ---  & $0.92752 \pm 0.00006$ & $0.63412 \pm 0.00010$ \\
 426.2   &    ---  &   ---  &   ---  & $0.92843 \pm 0.00013$ & $0.63669 \pm 0.00015$ \\
 427.5   &    ---  &   ---  & $0.33676 \pm 0.00005$ & $0.93108 \pm 0.00012$ & $0.63591 \pm 0.00088$ \\
 430.3   &  $0.87284 \pm 0.00054$ &   ---  &   ---  &   ---  & $0.63566 \pm 0.00065$ \\
 434.2   &    ---  & $0.66491 \pm 0.00036$ &   ---  &   ---  & $0.63455 \pm 0.00030$ \\
 436.5   &    ---  &   ---  & $0.33652 \pm 0.00024$ & $0.92902 \pm 0.00015$ & $0.63339 \pm 0.00038$ \\
 439.2   &    ---  &   ---  & $0.33889 \pm 0.00020$ & $0.92774 \pm 0.00017$ & $0.63584 \pm 0.00025$ \\
 440.6   &    ---  &   ---  & $0.33504 \pm 0.00009$ & $0.92750 \pm 0.00008$ & $0.63349 \pm 0.00021$ \\
 451.5   &  $0.87512 \pm 0.00008$ & $0.66494 \pm 0.00014$ & $0.33571 \pm 0.00003$ & $0.92845 \pm 0.00003$ & $0.63488 \pm 0.00005$ \\
 452.4   &  $0.87200 \pm 0.00014$ & $0.66303 \pm 0.00026$ & $0.33775 \pm 0.00003$ & $0.93009 \pm 0.00004$ & $0.63377 \pm 0.00006$ \\
 453.2   &  $0.87205 \pm 0.00025$ &   ---  &   ---  & $0.92972 \pm 0.00007$ & $0.63572 \pm 0.00011$ \\
 493.7   &  $0.87324 \pm 0.00008$ & $0.66474 \pm 0.00014$ & $0.33963 \pm 0.00003$ & $0.92712 \pm 0.00004$ &   ---  \\
 494.8   &  $0.87117 \pm 0.00017$ &   ---  & $0.33761 \pm 0.00024$ & $0.93116 \pm 0.00016$ &   ---  \\
 511.9   &    ---  &   ---  & $0.33664 \pm 0.00038$ & $0.93201 \pm 0.00021$ &   ---  \\
 515.0   &  $0.87294 \pm 0.00044$ & $0.66586 \pm 0.00033$ &   ---  & $0.93209 \pm 0.00024$ & $0.63449 \pm 0.00028$ \\
 516.0   &  $0.87372 \pm 0.00005$ & $0.66170 \pm 0.00007$ & $0.33459 \pm 0.00002$ & $0.93114 \pm 0.00002$ & $0.63793 \pm 0.00003$ \\
 517.1   &  $0.87691 \pm 0.00032$ & $0.66699 \pm 0.00015$ & $0.33920 \pm 0.00003$ & $0.92917 \pm 0.00003$ &   ---  \\
 518.2   &    ---  &   ---  & $0.33511 \pm 0.00004$ & $0.93082 \pm 0.00005$ & $0.63406 \pm 0.00011$ \\
 526.4   &    ---  &   ---  & $0.33850 \pm 0.00071$ &   ---  & $0.63805 \pm 0.00023$ \\
 536.9   &  $0.87173 \pm 0.00042$ &   ---  & $0.33814 \pm 0.00009$ & $0.93110 \pm 0.00025$ & $0.63381 \pm 0.00017$ \\
 538.1   &  $0.87275 \pm 0.00011$ &   ---  & $0.33642 \pm 0.00003$ &   ---  & $0.63521 \pm 0.00006$ \\
 539.3   &  $0.87729 \pm 0.00008$ & $0.66635 \pm 0.00009$ & $0.33895 \pm 0.00002$ & $0.92931 \pm 0.00002$ &   ---  \\
 540.9   &    ---  &   ---  &   ---  & $0.93062 \pm 0.00024$ & $0.63618 \pm 0.00081$ \\
 544.3   &    ---  &   ---  &   ---  & $0.93033 \pm 0.00032$ & $0.63435 \pm 0.00032$ \\
 557.1   &    ---  &   ---  & $0.33598 \pm 0.00004$ & $0.92978 \pm 0.00021$ & $0.63656 \pm 0.00018$ \\
 558.4   &    ---  &   ---  & $0.33760 \pm 0.00005$ & $0.92676 \pm 0.00011$ & $0.63715 \pm 0.00009$ \\
 559.7   &    ---  &   ---  & $0.33669 \pm 0.00015$ & $0.92945 \pm 0.00012$ & $0.63793 \pm 0.00034$ \\
 561.9   &  $0.87590 \pm 0.00037$ &   ---  &   ---  & $0.93013 \pm 0.00034$ & $0.63311 \pm 0.00034$ \\
 641.4   &    ---  &   ---  & $0.34081 \pm 0.00014$ & $0.92877 \pm 0.00044$ &   ---  \\
 644.9   &    ---  & $0.66237 \pm 0.00035$ & $0.33496 \pm 0.00017$ &   ---  &   ---  \\
 668.5   &    ---  &   ---  & $0.34061 \pm 0.00044$ &   ---  & $0.63354 \pm 0.00064$ \\
 685.8   &    ---  &   ---  & $0.33836 \pm 0.00087$ & $0.92913 \pm 0.00043$ &   ---  \\
 689.7   &    ---  &   ---  & $0.33623 \pm 0.00031$ & $0.92719 \pm 0.00029$ &   ---  \\
 705.8   &    ---  & $0.66324 \pm 0.00070$ & $0.33805 \pm 0.00021$ &   ---  &   ---  \\
 727.0   &    ---  &   ---  & $0.33447 \pm 0.00023$ &   ---  & $0.64047 \pm 0.00043$ \\
 729.6   &    ---  &   ---  & $0.33716 \pm 0.00056$ & $0.92776 \pm 0.00048$ &   ---  \\
 731.6   &    ---  &   ---  & $0.34265 \pm 0.00017$ & $0.92821 \pm 0.00033$ & $0.63376 \pm 0.00071$ \\
 755.3   &    ---  &   ---  & $0.34046 \pm 0.00056$ & $0.93002 \pm 0.00056$ &   ---  \\
 812.5   &    ---  & $0.66364 \pm 0.00081$ & $0.33798 \pm 0.00044$ &   ---  &   ---  \\
 819.7   &  $0.88000 \pm 0.00044$ &   ---  & $0.34294 \pm 0.00023$ & $0.93255 \pm 0.00030$ &   ---  \\
 842.8   &  $0.87684 \pm 0.00028$ &   ---  & $0.34161 \pm 0.00020$ &   ---  &   ---  \\
 861.7   &    ---  & $0.66356 \pm 0.00057$ &   ---  & $0.93410 \pm 0.00029$ &   ---  \\
 877.6   &    ---  &   ---  &   ---  & $0.92911 \pm 0.00069$ & $0.64155 \pm 0.00055$ \\

        &      &      &      &      &      \\ \hline
 \end{tabular}



==> 9118tb4L.tex <==
% Tabela com as amplitudes para cada ano.

 % TABLE - Amplitudes

 \begin{longtable} {cccccc}
 \caption{ Observed amplitudes (in mma) in each data set.} \\
\hline \hline
Mode  & 1983 & 1985 & 1989 & 1993 & 2002 \\
 (s)      &        &         &        &         &      \\ \hline
Period (s)   &        &         &        &         &      \\ 
             &        &         &        &         &      \\ 
\endfirsthead
\caption{continued.}\\
\hline \hline
Mode  & 1983 & 1985 & 1989 & 1993 & 2002 \\
 (s)      &        &         &        &         &      \\ \hline
Period (s)   &        &         &        &         &      \\ 
             &        &         &        &         &      \\ 
\endhead
\hline
\endfoot
 376.0   &  $ 0.72 \pm 0.13$ & $ 0.35 \pm 0.19$ &   ---  &   ---  &   ---  \\
 387.4   &    ---  &   ---  & $ 0.30 \pm 0.05$ &   ---  & $ 0.43 \pm 0.09$ \\
 390.3   &  $ 1.77 \pm 0.13$ &   ---  & $ 1.01 \pm 0.05$ &   ---  & $ 0.22 \pm 0.09$ \\
 390.8   &    ---  &   ---  &   ---  & $ 0.28 \pm 0.07$ & $ 0.15 \pm 0.09$ \\
 397.2   &    ---  & $ 0.49 \pm 0.17$ &   ---  &   ---  & $ 0.33 \pm 0.09$ \\
 399.0   &    ---  &   ---  & $ 0.37 \pm 0.05$ &   ---  & $ 0.66 \pm 0.09$ \\
 400.0   &    ---  &   ---  & $ 1.42 \pm 0.05$ & $ 0.79 \pm 0.07$ & $ 0.61 \pm 0.09$ \\
 401.6   &    ---  &   ---  &   ---  &   ---  & $ 0.38 \pm 0.09$ \\
 412.0   &    ---  &   ---  & $ 0.60 \pm 0.05$ &   ---  & $ 0.64 \pm 0.09$ \\
 414.3   &    ---  &   ---  & $ 0.65 \pm 0.05$ & $ 0.56 \pm 0.07$ & $ 0.70 \pm 0.09$ \\
 415.5   &    ---  & $ 0.81 \pm 0.18$ & $ 1.19 \pm 0.05$ &   ---  & $ 0.51 \pm 0.09$ \\
 422.5   &  $ 2.36 \pm 0.13$ &   ---  &   ---  & $ 1.82 \pm 0.07$ & $ 1.64 \pm 0.09$ \\
 426.2   &    ---  &   ---  &   ---  & $ 0.80 \pm 0.07$ & $ 0.98 \pm 0.09$ \\
 427.5   &    ---  &   ---  & $ 1.92 \pm 0.05$ & $ 0.85 \pm 0.07$ & $ 0.16 \pm 0.09$ \\
 430.3   &  $ 0.61 \pm 0.14$ &   ---  &   ---  &   ---  & $ 0.24 \pm 0.09$ \\
 434.2   &    ---  & $ 0.88 \pm 0.19$ &   ---  &   ---  & $ 0.48 \pm 0.09$ \\
 436.5   &    ---  &   ---  & $ 0.41 \pm 0.05$ & $ 0.72 \pm 0.07$ & $ 0.39 \pm 0.09$ \\
 439.2   &    ---  &   ---  & $ 0.49 \pm 0.05$ & $ 0.61 \pm 0.07$ & $ 0.60 \pm 0.09$ \\
 440.6   &    ---  &   ---  & $ 1.05 \pm 0.05$ & $ 1.26 \pm 0.07$ & $ 0.72 \pm 0.09$ \\
 451.5   &  $ 4.54 \pm 0.15$ & $ 2.72 \pm 0.21$ & $ 3.70 \pm 0.05$ & $ 3.93 \pm 0.07$ & $ 3.39 \pm 0.09$ \\
 452.4   &  $ 2.78 \pm 0.15$ & $ 1.37 \pm 0.20$ & $ 3.36 \pm 0.05$ & $ 2.80 \pm 0.07$ & $ 2.78 \pm 0.09$ \\
 453.2   &  $ 1.41 \pm 0.14$ &   ---  &   ---  & $ 1.56 \pm 0.07$ & $ 1.47 \pm 0.09$ \\
 493.7   &  $ 5.47 \pm 0.16$ & $ 3.00 \pm 0.22$ & $ 3.47 \pm 0.05$ & $ 2.75 \pm 0.07$ &   ---  \\
 494.8   &  $ 2.34 \pm 0.15$ &   ---  & $ 0.46 \pm 0.05$ & $ 0.72 \pm 0.07$ &   ---  \\
 511.9   &    ---  &   ---  & $ 0.29 \pm 0.05$ & $ 0.59 \pm 0.07$ &   ---  \\
 515.0   &  $ 0.91 \pm 0.14$ & $ 1.21 \pm 0.20$ &   ---  & $ 0.58 \pm 0.07$ & $ 0.69 \pm 0.09$ \\
 516.0   &  $ 8.76 \pm 0.16$ & $ 7.45 \pm 0.24$ & $ 6.17 \pm 0.06$ & $ 5.91 \pm 0.08$ & $ 7.25 \pm 0.09$ \\
 517.1   &  $ 1.30 \pm 0.15$ & $ 3.01 \pm 0.22$ & $ 3.89 \pm 0.05$ & $ 4.26 \pm 0.08$ &   ---  \\
 518.2   &    ---  &   ---  & $ 3.58 \pm 0.06$ & $ 3.12 \pm 0.08$ & $ 1.71 \pm 0.09$ \\
 526.4   &    ---  &   ---  & $ 0.16 \pm 0.05$ &   ---  & $ 0.77 \pm 0.09$ \\
 536.9   &  $ 1.01 \pm 0.14$ &   ---  & $ 1.41 \pm 0.06$ & $ 0.52 \pm 0.07$ & $ 1.16 \pm 0.10$ \\
 538.1   &  $ 4.48 \pm 0.16$ &   ---  & $ 3.82 \pm 0.05$ &   ---  & $ 2.98 \pm 0.09$ \\
 539.3   &  $ 5.93 \pm 0.16$ & $ 4.48 \pm 0.20$ & $ 5.37 \pm 0.06$ & $ 7.47 \pm 0.08$ &   ---  \\
 540.9   &    ---  &   ---  &   ---  & $ 0.55 \pm 0.07$ & $ 0.23 \pm 0.09$ \\
 544.3   &    ---  &   ---  &   ---  & $ 0.41 \pm 0.07$ & $ 0.63 \pm 0.10$ \\
 557.1   &    ---  &   ---  & $ 3.14 \pm 0.05$ & $ 0.69 \pm 0.08$ & $ 1.04 \pm 0.09$ \\
 558.4   &    ---  &   ---  & $ 2.49 \pm 0.05$ & $ 1.51 \pm 0.08$ & $ 2.22 \pm 0.09$ \\
 559.7   &    ---  &   ---  & $ 0.84 \pm 0.05$ & $ 1.38 \pm 0.08$ & $ 0.56 \pm 0.09$ \\
 561.9   &  $ 1.21 \pm 0.15$ &   ---  &   ---  & $ 0.43 \pm 0.08$ & $ 0.55 \pm 0.09$ \\
 641.4   &    ---  &   ---  & $ 1.03 \pm 0.05$ & $ 0.35 \pm 0.07$ &   ---  \\
 644.9   &    ---  & $ 1.75 \pm 0.24$ & $ 0.87 \pm 0.05$ &   ---  &   ---  \\
 668.5   &    ---  &   ---  & $ 0.35 \pm 0.05$ &   ---  & $ 0.35 \pm 0.09$ \\
 685.8   &    ---  &   ---  & $ 0.17 \pm 0.05$ & $ 0.39 \pm 0.07$ &   ---  \\
 689.7   &    ---  &   ---  & $ 0.51 \pm 0.05$ & $ 0.60 \pm 0.07$ &   ---  \\
 705.8   &    ---  & $ 0.76 \pm 0.19$ & $ 0.75 \pm 0.05$ &   ---  &   ---  \\
 727.0   &    ---  &   ---  & $ 0.72 \pm 0.05$ &   ---  & $ 0.60 \pm 0.09$ \\
 729.6   &    ---  &   ---  & $ 0.29 \pm 0.05$ & $ 0.36 \pm 0.07$ &   ---  \\
 731.6   &    ---  &   ---  & $ 0.98 \pm 0.05$ & $ 0.55 \pm 0.07$ & $ 0.34 \pm 0.09$ \\
 755.3   &    ---  &   ---  & $ 0.31 \pm 0.05$ & $ 0.33 \pm 0.07$ &   ---  \\
 812.5   &    ---  & $ 0.73 \pm 0.18$ & $ 0.41 \pm 0.05$ &   ---  &   ---  \\
 819.7   &  $ 1.40 \pm 0.14$ &   ---  & $ 0.81 \pm 0.05$ & $ 0.65 \pm 0.07$ &   ---  \\
 842.8   &  $ 2.28 \pm 0.14$ &   ---  & $ 0.91 \pm 0.05$ &   ---  &   ---  \\
 861.7   &    ---  & $ 1.09 \pm 0.18$ &   ---  & $ 0.72 \pm 0.07$ &   ---  \\
 877.6   &    ---  &   ---  &   ---  & $ 0.30 \pm 0.07$ & $ 0.53 \pm 0.09$ \\

        &      &      &      &      &      \\ \hline
  \end{longtable}




==> 9118tb5L.tex <==

% TABLE - Time of maximum.

 \begin{longtable} {cccccc}
 \caption{ Observed times of maximum (in BCT) in each data set. } \\
\hline \hline
Year    & 1983 & 1985 & 1989 & 1993 & 2002 \\
BCT     & $ 244\,5346.0+$      & $ 244\,6147.0+$       & $ 244\,7593.0+$      &  $ 244\,9065.0+$      & $ 245\,2410.0+$    \\ \hline
Period (s)   &        &         &        &         &      \\ 
             &        &         &        &         &      \\ 
\endfirsthead
\caption{continued.}\\
\hline \hline
Year    & 1983 & 1985 & 1989 & 1993 & 2002 \\
BCT     & $ 244\,5346.0+$      & $ 244\,6147.0+$       & $ 244\,7593.0+$      &  $ 244\,9065.0+$      & $ 245\,2410.0+$    \\ \hline
Period (s)   &        &         &        &         &      \\ 
             &        &         &        &         &      \\ 
\endhead
\hline
\endfoot

 376.0   &  $0.87548 \pm 0.00038$ & $0.66449 \pm 0.00079$ &   ---  &   ---  &   ---  \\
 387.4   &    ---  &   ---  & $0.33622 \pm 0.00028$ &   ---  & $0.63362 \pm 0.00030$ \\
 390.3   &  $0.87395 \pm 0.00016$ &   ---  & $0.33753 \pm 0.00009$ &   ---  & $0.63347 \pm 0.00059$ \\
 390.8   &    ---  &   ---  &   ---  & $0.92851 \pm 0.00034$ & $0.63559 \pm 0.00090$ \\
 397.2   &    ---  & $0.66570 \pm 0.00055$ &   ---  &   ---  & $0.63552 \pm 0.00042$ \\
 399.0   &    ---  &   ---  & $0.33756 \pm 0.00023$ &   ---  & $0.63368 \pm 0.00020$ \\
 400.0   &    ---  &   ---  & $0.33522 \pm 0.00006$ & $0.92791 \pm 0.00012$ & $0.63537 \pm 0.00022$ \\
 401.6   &    ---  &   ---  &   ---  &   ---  & $0.63608 \pm 0.00037$ \\
 412.0   &    ---  &   ---  & $0.33584 \pm 0.00015$ &   ---  & $0.63361 \pm 0.00022$ \\
 414.3   &    ---  &   ---  & $0.33513 \pm 0.00015$ & $0.92697 \pm 0.00018$ & $0.63441 \pm 0.00020$ \\
 415.5   &    ---  & $0.66172 \pm 0.00037$ & $0.33537 \pm 0.00008$ &   ---  & $0.63412 \pm 0.00027$ \\
 422.5   &  $0.87207 \pm 0.00013$ &   ---  &   ---  & $0.92752 \pm 0.00006$ & $0.63412 \pm 0.00010$ \\
 426.2   &    ---  &   ---  &   ---  & $0.92843 \pm 0.00013$ & $0.63669 \pm 0.00015$ \\
 427.5   &    ---  &   ---  & $0.33676 \pm 0.00005$ & $0.93108 \pm 0.00012$ & $0.63591 \pm 0.00088$ \\
 430.3   &  $0.87284 \pm 0.00054$ &   ---  &   ---  &   ---  & $0.63566 \pm 0.00065$ \\
 434.2   &    ---  & $0.66491 \pm 0.00036$ &   ---  &   ---  & $0.63455 \pm 0.00030$ \\
 436.5   &    ---  &   ---  & $0.33652 \pm 0.00024$ & $0.92902 \pm 0.00015$ & $0.63339 \pm 0.00038$ \\
 439.2   &    ---  &   ---  & $0.33889 \pm 0.00020$ & $0.92774 \pm 0.00017$ & $0.63584 \pm 0.00025$ \\
 440.6   &    ---  &   ---  & $0.33504 \pm 0.00009$ & $0.92750 \pm 0.00008$ & $0.63349 \pm 0.00021$ \\
 451.5   &  $0.87512 \pm 0.00008$ & $0.66494 \pm 0.00014$ & $0.33571 \pm 0.00003$ & $0.92845 \pm 0.00003$ & $0.63488 \pm 0.00005$ \\
 452.4   &  $0.87200 \pm 0.00014$ & $0.66303 \pm 0.00026$ & $0.33775 \pm 0.00003$ & $0.93009 \pm 0.00004$ & $0.63377 \pm 0.00006$ \\
 453.2   &  $0.87205 \pm 0.00025$ &   ---  &   ---  & $0.92972 \pm 0.00007$ & $0.63572 \pm 0.00011$ \\
 493.7   &  $0.87324 \pm 0.00008$ & $0.66474 \pm 0.00014$ & $0.33963 \pm 0.00003$ & $0.92712 \pm 0.00004$ &   ---  \\
 494.8   &  $0.87117 \pm 0.00017$ &   ---  & $0.33761 \pm 0.00024$ & $0.93116 \pm 0.00016$ &   ---  \\
 511.9   &    ---  &   ---  & $0.33664 \pm 0.00038$ & $0.93201 \pm 0.00021$ &   ---  \\
 515.0   &  $0.87294 \pm 0.00044$ & $0.66586 \pm 0.00033$ &   ---  & $0.93209 \pm 0.00024$ & $0.63449 \pm 0.00028$ \\
 516.0   &  $0.87372 \pm 0.00005$ & $0.66170 \pm 0.00007$ & $0.33459 \pm 0.00002$ & $0.93114 \pm 0.00002$ & $0.63793 \pm 0.00003$ \\
 517.1   &  $0.87691 \pm 0.00032$ & $0.66699 \pm 0.00015$ & $0.33920 \pm 0.00003$ & $0.92917 \pm 0.00003$ &   ---  \\
 518.2   &    ---  &   ---  & $0.33511 \pm 0.00004$ & $0.93082 \pm 0.00005$ & $0.63406 \pm 0.00011$ \\
 526.4   &    ---  &   ---  & $0.33850 \pm 0.00071$ &   ---  & $0.63805 \pm 0.00023$ \\
 536.9   &  $0.87173 \pm 0.00042$ &   ---  & $0.33814 \pm 0.00009$ & $0.93110 \pm 0.00025$ & $0.63381 \pm 0.00017$ \\
 538.1   &  $0.87275 \pm 0.00011$ &   ---  & $0.33642 \pm 0.00003$ &   ---  & $0.63521 \pm 0.00006$ \\
 539.3   &  $0.87729 \pm 0.00008$ & $0.66635 \pm 0.00009$ & $0.33895 \pm 0.00002$ & $0.92931 \pm 0.00002$ &   ---  \\
 540.9   &    ---  &   ---  &   ---  & $0.93062 \pm 0.00024$ & $0.63618 \pm 0.00081$ \\
 544.3   &    ---  &   ---  &   ---  & $0.93033 \pm 0.00032$ & $0.63435 \pm 0.00032$ \\
 557.1   &    ---  &   ---  & $0.33598 \pm 0.00004$ & $0.92978 \pm 0.00021$ & $0.63656 \pm 0.00018$ \\
 558.4   &    ---  &   ---  & $0.33760 \pm 0.00005$ & $0.92676 \pm 0.00011$ & $0.63715 \pm 0.00009$ \\
 559.7   &    ---  &   ---  & $0.33669 \pm 0.00015$ & $0.92945 \pm 0.00012$ & $0.63793 \pm 0.00034$ \\
 561.9   &  $0.87590 \pm 0.00037$ &   ---  &   ---  & $0.93013 \pm 0.00034$ & $0.63311 \pm 0.00034$ \\
 641.4   &    ---  &   ---  & $0.34081 \pm 0.00014$ & $0.92877 \pm 0.00044$ &   ---  \\
 644.9   &    ---  & $0.66237 \pm 0.00035$ & $0.33496 \pm 0.00017$ &   ---  &   ---  \\
 668.5   &    ---  &   ---  & $0.34061 \pm 0.00044$ &   ---  & $0.63354 \pm 0.00064$ \\
 685.8   &    ---  &   ---  & $0.33836 \pm 0.00087$ & $0.92913 \pm 0.00043$ &   ---  \\
 689.7   &    ---  &   ---  & $0.33623 \pm 0.00031$ & $0.92719 \pm 0.00029$ &   ---  \\
 705.8   &    ---  & $0.66324 \pm 0.00070$ & $0.33805 \pm 0.00021$ &   ---  &   ---  \\
 727.0   &    ---  &   ---  & $0.33447 \pm 0.00023$ &   ---  & $0.64047 \pm 0.00043$ \\
 729.6   &    ---  &   ---  & $0.33716 \pm 0.00056$ & $0.92776 \pm 0.00048$ &   ---  \\
 731.6   &    ---  &   ---  & $0.34265 \pm 0.00017$ & $0.92821 \pm 0.00033$ & $0.63376 \pm 0.00071$ \\
 755.3   &    ---  &   ---  & $0.34046 \pm 0.00056$ & $0.93002 \pm 0.00056$ &   ---  \\
 812.5   &    ---  & $0.66364 \pm 0.00081$ & $0.33798 \pm 0.00044$ &   ---  &   ---  \\
 819.7   &  $0.88000 \pm 0.00044$ &   ---  & $0.34294 \pm 0.00023$ & $0.93255 \pm 0.00030$ &   ---  \\
 842.8   &  $0.87684 \pm 0.00028$ &   ---  & $0.34161 \pm 0.00020$ &   ---  &   ---  \\
 861.7   &    ---  & $0.66356 \pm 0.00057$ &   ---  & $0.93410 \pm 0.00029$ &   ---  \\
 877.6   &    ---  &   ---  &   ---  & $0.92911 \pm 0.00069$ & $0.64155 \pm 0.00055$ \\

        &      &      &      &      &      \\ \hline
 \end{longtable}



